STRING: A Schema-Thinking Robot Agent That Learns from Embodied Experience in a Multiphysics World

Dexterous robots usually learn deformable, contact-rich tasks from teleoperated demonstrations, and the resulting policy works only where the data reached. Robot agents built on large language models need no such data, but they accumulate skills that overfit to the task they were found on. We argue that an agent is all you need for dexterous manipulation if it learns as people do, by abstracting physical schemas from embodied experience instead of collecting skills. We present STRING, a system in which a schema-based robot agent gains this experience in STRING World, a multiphysics engine we built from scratch. STRING World gives each class of material its own solver, from elastic solids and thin shells to fracturing, granular and liquid matter, strings with audio, and air, and simulates them together with the robot in one scene, covering more kinds of matter than simulators such as MuJoCo and Isaac Sim. It returns the physical quantities it computes, such as contact reactions and solver state, to the agent as observables. From one human demonstration, the agent rehearses the task in STRING World and abstracts physical schemas, whose roles, relations, phases and force ranges are predicates over the observables. The schemas and their subgoals carry from simulation to reality, where the robot reproduces the task from a real-time 3D reconstruction of the scene, with no teleoperation data or policy network. On a bimanual dexterous robot, STRING reaches 50.0% average success over ten tasks, from knotting a rope to flying a paper plane with a hair dryer, against 2.5% for the best general-purpose agent given the same demonstration and STRING World. On the four hardest tasks it reaches 43.8%, against 27.5% for the best fine-tuned policy.

==> sections/icons_schema.tex <==
\definecolor{scRope}{RGB}{214,40,44}
\definecolor{scRopeD}{RGB}{140,18,26}
\definecolor{scPad}{RGB}{214,218,225}
\definecolor{scBlock}{RGB}{251,227,210}
\newcommand{\scPad}{\filldraw[sl, fill=scPad, rounded corners=0.5pt] (-0.18,-0.08) rectangle (0.18,0.08); \draw[line width=0.25pt, draw=fgSub!70] (-0.10,0.025) -- (0.10,0.025);}
\newcommand{\scPadDash}{\draw[line width=0.40pt, draw=fgSub!80, dash pattern=on 0.9pt off 0.7pt, rounded corners=0.5pt] (-0.18,-0.08) rectangle (0.18,0.08);}
\newcommand{\scTable}{\draw[sl] (0.02,0) -- (0.98,0); \foreach \u in {0.16,0.34,0.52,0.70,0.88} \draw[line width=0.28pt, draw=fgInk] (\u,0) -- (\u-0.09,-0.09);}
\tikzset{
  sl/.style={line width=0.40pt, line cap=round, line join=round, draw=fgInk},
  sg/.style={line width=0.40pt, line cap=round, draw=fgSub!80},
  sup/.style={line width=0.55pt, draw=fgHi, -{Stealth[length=2.0pt, width=2.1pt]}},
  sgr/.style={line width=0.45pt, draw=fgSub!85, -{Stealth[length=1.7pt, width=1.8pt]}},
  sbl/.style={line width=0.55pt, draw=fgBlueD, -{Stealth[length=2.0pt, width=2.1pt]}},
  ropeO/.style={line width=#1*1.35pt, draw=scRopeD, line cap=round},
  ropeI/.style={line width=#1pt, draw=scRope, line cap=round},
  pics/evLiftStalls/.style={code={
    \draw[ropeO=1.0] (0.06,0.36) .. controls (0.30,0.50) and (0.70,0.50) .. (0.94,0.36);
    \draw[ropeI=1.0] (0.06,0.36) .. controls (0.30,0.50) and (0.70,0.50) .. (0.94,0.36);
    \begin{scope}[shift={(0.50,0.31)}]\scPad\end{scope}
    \draw[sup] (0.50,0.56) -- (0.50,0.84);
    \draw[line width=0.75pt, draw=fgInk] (0.36,0.90) -- (0.64,0.90);}},
  pics/evLiftSupported/.style={code={
    \draw[ropeO=1.0] (0.04,0.22) .. controls (0.30,0.70) and (0.70,0.70) .. (0.96,0.22);
    \draw[ropeI=1.0] (0.04,0.22) .. controls (0.30,0.70) and (0.70,0.70) .. (0.96,0.22);
    \begin{scope}[shift={(0.50,0.48)}]\scPad\end{scope}
    \draw[sup] (0.50,0.66) -- (0.50,0.98);}},
  pics/evGripLost/.style={code={
    \begin{scope}[shift={(0.26,0.70)}, rotate=90]\scPad\end{scope} \begin{scope}[shift={(0.74,0.70)}, rotate=90]\scPad\end{scope}
    \draw[line width=0.4pt, draw=fgSub!80, dash pattern=on 0.8pt off 0.6pt] (0.50,0.70) circle (0.15);
    \filldraw[line width=0.5pt, draw=scRopeD, fill=scRope] (0.50,0.16) circle (0.13);
    \draw[sup] (0.50,0.52) -- (0.50,0.33);}},
  pics/evContactShifts/.style={code={
    \fill[scRope!25] (0.04,0.30) rectangle (0.36,0.48); \fill[scRope!55] (0.36,0.30) rectangle (0.68,0.48); \fill[scRope!25] (0.68,0.30) rectangle (0.96,0.48);
    \draw[line width=0.4pt, draw=scRopeD] (0.04,0.30) rectangle (0.96,0.48);
    \begin{scope}[shift={(0.20,0.58)}]\scPadDash\end{scope} \begin{scope}[shift={(0.80,0.58)}]\scPad\end{scope}
    \draw[sup] (0.28,0.80) .. controls (0.42,0.98) and (0.58,0.98) .. (0.72,0.80);}},
  pics/evLoadTransfer/.style={code={
    \begin{scope}[shift={(0,0.18)}]\scTable\end{scope}
    \filldraw[line width=0.5pt, draw=scRopeD, fill=scRope] (0.50,0.31) ellipse (0.24 and 0.12);
    \begin{scope}[shift={(0.50,0.52)}]\scPad\end{scope}
    \draw[sgr] (0.50,0.94) -- (0.50,0.64);
    \draw[sup] (0.16,0.02) -- (0.16,0.42); \draw[sup] (0.84,0.02) -- (0.84,0.42);}},
  pics/evHandRelease/.style={code={
    \begin{scope}[shift={(0,0.18)}]\scTable\end{scope}
    \filldraw[line width=0.5pt, draw=scRopeD, fill=scRope] (0.50,0.31) ellipse (0.24 and 0.12);
    \begin{scope}[shift={(0.50,0.52)}]\scPadDash\end{scope}
    \begin{scope}[shift={(0.50,0.76)}]\scPad\end{scope}
    \draw[sup] (0.80,0.56) -- (0.80,0.96);}},
  pics/evBendingBuilds/.style={code={
    \filldraw[line width=0.45pt, draw=fgInk, fill=white] (0.10,0.30) .. controls (0.35,0.62) and (0.65,0.62) .. (0.90,0.30) -- (0.90,0.22) .. controls (0.65,0.54) and (0.35,0.54) .. (0.10,0.22) -- cycle;
    \draw[sbl] (0.06,0.62) .. controls (0.10,0.46) .. (0.18,0.40);
    \draw[sbl] (0.94,0.62) .. controls (0.90,0.46) .. (0.82,0.40);
    \fill[scRope] (0.50,0.48) circle (0.035);}},
  pics/evBendingRelaxes/.style={code={
    \draw[line width=0.40pt, draw=fgSub!80, dash pattern=on 0.8pt off 0.6pt] (0.10,0.40) .. controls (0.35,0.72) and (0.65,0.72) .. (0.90,0.40);
    \filldraw[line width=0.45pt, draw=fgInk, fill=white] (0.08,0.26) rectangle (0.92,0.34);
    \fill[scRope] (0.50,0.30) circle (0.035);
    \draw[sbl] (0.30,0.60) -- (0.30,0.40); \draw[sbl] (0.70,0.60) -- (0.70,0.40);}},
  pics/scDirectionalSupport/.style={code={
    \filldraw[line width=0.6pt, draw=scRopeD, fill=scRope] (0.50,0.58) circle (0.15);
    \fill[white, opacity=0.55] (0.46,0.62) circle (0.045);
    \begin{scope}[shift={(0.50,0.36)}, scale=1.25]\scPad\end{scope}
    \draw[sup, line width=0.8pt] (0.50,0.02) -- (0.50,0.25);
    \draw[sgr] (0.04,0.58) -- (0.28,0.58); \draw[sgr] (0.96,0.58) -- (0.72,0.58);
    \draw[line width=0.5pt, draw=fgSub!85] (0.10,0.80) -- (0.22,0.70) (0.78,0.80) -- (0.90,0.70);}},
  pics/scContactIdentity/.style={code={
    \fill[scRope!22] (0.03,0.36) rectangle (0.35,0.56); \fill[scRope!60] (0.35,0.36) rectangle (0.65,0.56); \fill[scRope!22] (0.65,0.36) rectangle (0.97,0.56);
    \draw[line width=0.45pt, draw=scRopeD] (0.03,0.36) rectangle (0.97,0.56);
    \draw[line width=0.3pt, draw=scRopeD] (0.35,0.36) -- (0.35,0.56) (0.65,0.36) -- (0.65,0.56);
    \begin{scope}[shift={(0.19,0.66)}, scale=1.15]\scPadDash\end{scope}
    \begin{scope}[shift={(0.81,0.66)}, scale=1.15]\scPad\end{scope}
    \begin{scope}[shift={(0.81,0.26)}, scale=1.15]\scPad\end{scope}
    \node[inner sep=0pt, font=\fontsize{6.5}{6}\selectfont\bfseries, text=fgHi] at (0.50,0.84) {$\neq$};}},
  pics/scSupportRedistribution/.style={code={
    \begin{scope}[shift={(0,0.16)}]\scTable\end{scope}
    \filldraw[line width=0.6pt, draw=scRopeD, fill=scRope] (0.42,0.30) ellipse (0.26 and 0.13);
    \fill[white, opacity=0.5] (0.36,0.34) ellipse (0.08 and 0.03);
    \draw[sup, line width=0.8pt] (0.16,-0.04) -- (0.16,0.36); \draw[sup, line width=0.8pt] (0.68,-0.04) -- (0.68,0.36);
    \begin{scope}[shift={(0.42,0.50)}, scale=1.15]\scPadDash\end{scope}
    \begin{scope}[shift={(0.42,0.80)}, scale=1.15]\scPad\end{scope}
    \draw[sgr] (0.82,0.58) -- (0.82,0.96);}},
}


==> sections/logo.tex <==
\definecolor{lgRope}{RGB}{214,40,44}
\definecolor{lgRopeD}{RGB}{128,14,22}
\definecolor{lgRopeL}{RGB}{255,150,128}
\newcommand{\stringknotpath}[2]{plot[domain=#1:#2, samples=90, smooth, variable=\t] ({sin(\t)+2*sin(2*\t)},{cos(\t)-2*cos(2*\t)})}
\tikzset{pics/stringknot/.style={code={%
  \pgfmathsetmacro\lgw{#1*3.6}%
  \begin{scope}[x={#1cm/5.4}, y={#1cm/5.4}, line cap=round, line join=round]
    \draw[lgRopeD, line width=\lgw pt] \stringknotpath{0}{360};
    \draw[lgRope, line width=0.74*\lgw pt] \stringknotpath{0}{360};
    \draw[lgRopeL, line width=0.16*\lgw pt, shift={(-0.06,0.07)}] \stringknotpath{0}{360};
    \foreach \c in {15.5,135.4,255.5}{
      \draw[white, line width=1.55*\lgw pt, line cap=butt] \stringknotpath{\c-15}{\c+15};
      \draw[lgRopeD, line width=\lgw pt, line cap=butt] \stringknotpath{\c-24}{\c+24};
      \draw[lgRope, line width=0.74*\lgw pt, line cap=butt] \stringknotpath{\c-25}{\c+25};
      \draw[lgRopeL, line width=0.16*\lgw pt, shift={(-0.06,0.07)}] \stringknotpath{\c-25}{\c+25};
    }
  \end{scope}}}}
\newcommand{\stringknot}[1]{\tikz[baseline={(0,{-0.41*#1})}]{\pic{stringknot=#1};}}

\definecolor{swAir}{RGB}{120,196,242}
\definecolor{swShell}{RGB}{150,112,224}
\definecolor{swLiquid}{RGB}{38,120,214}
\definecolor{swGrain}{RGB}{52,184,150}
\definecolor{swSolid}{RGB}{244,150,44}
\tikzset{pics/stringworld/.style={code={%
  \pgfmathsetmacro\swr{#1/2}%
  \pgfmathsetmacro\swl{#1*2.2}%
  \begin{scope}[x=\swr cm, y=\swr cm, line cap=round, line join=round]
    \begin{scope}[rotate=-16]
      \draw[lgRopeD, line width=\swl pt] (1.42,0) arc[start angle=0, end angle=180, x radius=1.42, y radius=0.40];
      \draw[lgRope, line width=0.66*\swl pt] (1.42,0) arc[start angle=0, end angle=180, x radius=1.42, y radius=0.40];
    \end{scope}
    \begin{scope}
      \clip (0,0) circle (1);
      \fill[swSolid] (-1,-1) rectangle (1,1);
      \foreach \y/\c in {-0.56/swGrain, -0.18/swLiquid, 0.20/swShell, 0.58/swAir}
        \fill[\c] (-1.1,\y) arc[start angle=180, end angle=360, x radius=1.1, y radius=0.24] -- (1.1,1.1) -- (-1.1,1.1) -- cycle;
      \foreach \y in {-0.56,-0.18,0.20,0.58}
        \draw[white, opacity=0.55, line width=0.10*\swl pt] (-1.1,\y) arc[start angle=180, end angle=360, x radius=1.1, y radius=0.24];
      \draw[white, opacity=0.55, line width=0.10*\swl pt] (0,-1) arc[start angle=-90, end angle=90, x radius=0.46, y radius=1] (0,1) arc[start angle=90, end angle=270, x radius=0.46, y radius=1];
      \fill[black, path fading=swRim] (0,0) circle (1);
      \fill[white, opacity=0.42, rotate=38] (-0.02,0.66) ellipse (0.34 and 0.17);
    \end{scope}
    \draw[white, line width=0.16*\swl pt] (0,0) circle (1);
    \begin{scope}[rotate=-16]
      \draw[lgRopeD, line width=\swl pt] (-1.42,0) arc[start angle=180, end angle=360, x radius=1.42, y radius=0.40];
      \draw[lgRope, line width=0.66*\swl pt] (-1.42,0) arc[start angle=180, end angle=360, x radius=1.42, y radius=0.40];
      \draw[lgRopeL, line width=0.14*\swl pt, shift={(0,0.025)}] (-1.30,-0.10) arc[start angle=195, end angle=330, x radius=1.42, y radius=0.40];
    \end{scope}
  \end{scope}}}}
\newcommand{\stringworld}[1]{\tikz[baseline={(0,{-0.36*#1})}]{\pic{stringworld=#1};}}

